Span-based discontinuous constituency parsing: a family of exact chart-based algorithms with time complexities from O(n^6) down to O(n^3)

We introduce a novel chart-based algorithm for span-based parsing of discontinuous constituency trees of block degree two, including ill-nested structures. In particular, we show that we can build variants of our parser with smaller search spaces and time complexities ranging from $\mathcal O(n^6)$ down to $\mathcal O(n^3)$. The cubic time variant covers 98\% of constituents observed in linguistic treebanks while having the same complexity as continuous constituency parsers. We evaluate our approach on German and English treebanks (Negra, Tiger and Discontinuous PTB) and report state-of-the-art results in the fully supervised setting. We also experiment with pre-trained word embeddings and \bert{}-based neural networks.

==> deductions/n3_combine.rule.tex <==
	$$
	\AxiomC{\scriptsize $[A, \top, i, -, -, m]$}
	\AxiomC{\scriptsize $[B, \top, m, -, -, j]$}
	\BinaryInfC{\scriptsize $[C, \top, i, -, -, j]$}
	\DisplayProof
	$$

==> recall.tex <==
\begin{tabular}{l|l|rclr|rclr|rclr|rclr|rclr}
 & & \multicolumn{4}{|c}{Continuous} & \multicolumn{4}{|c}{N4} & \multicolumn{4}{|c}{N5} & \multicolumn{4}{|c}{Well-nested} & \multicolumn{4}{|c}{Ill-nested} \\
\hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{dptb (dev)}}}
& bd2 & 28476 & / & 28925 & (98.45\%) & 28817 & / & 28925 & (99.63\%) & 28920 & / & 28925 & (99.98\%) & 28920 & / & 28925 & (99.98\%) & 28925 & / & 28925 & (100.00\%)\\
&- disc & 0 & / & 449 & (0.00\%) & 341 & / & 449 & (75.95\%) & 444 & / & 449 & (98.89\%) & 444 & / & 449 & (98.89\%) & 449 & / & 449 & (100.00\%)\\
& all & 28476 & / & 28950 & (98.36\%) & 28817 & / & 28950 & (99.54\%) & 28920 & / & 28950 & (99.90\%) & 28920 & / & 28950 & (99.90\%) & 28925 & / & 28950 & (99.91\%)\\
&- disc & 0 & / & 474 & (0.00\%) & 341 & / & 474 & (71.94\%) & 444 & / & 474 & (93.67\%) & 444 & / & 474 & (93.67\%) & 449 & / & 474 & (94.73\%)\\
\hline
& Total time (min)& \multicolumn{4}{|r}{0.000283333}& \multicolumn{4}{|r}{0.0394333}& \multicolumn{4}{|r}{0.141517}& \multicolumn{4}{|r}{0.621667}& \multicolumn{4}{|r}{0.673333}\\
& Sentences / min& \multicolumn{4}{|r}{6000000.0}& \multicolumn{4}{|r}{43110.7}& \multicolumn{4}{|r}{12012.7}& \multicolumn{4}{|r}{2734.58}& \multicolumn{4}{|r}{2524.75}\\
& Tokens / min& \multicolumn{4}{|r}{141589000.0}& \multicolumn{4}{|r}{1017340.0}& \multicolumn{4}{|r}{283479.0}& \multicolumn{4}{|r}{64531.4}& \multicolumn{4}{|r}{59579.7}\\
\hline
\hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{dptb (test)}}}
& bd2 & 40913 & / & 41670 & (98.18\%) & 41502 & / & 41670 & (99.60\%) & 41658 & / & 41670 & (99.97\%) & 41658 & / & 41670 & (99.97\%) & 41670 & / & 41670 & (100.00\%)\\
&- disc & 0 & / & 757 & (0.00\%) & 589 & / & 757 & (77.81\%) & 745 & / & 757 & (98.41\%) & 745 & / & 757 & (98.41\%) & 757 & / & 757 & (100.00\%)\\
& all & 40913 & / & 41767 & (97.96\%) & 41502 & / & 41767 & (99.37\%) & 41658 & / & 41767 & (99.74\%) & 41658 & / & 41767 & (99.74\%) & 41670 & / & 41767 & (99.77\%)\\
&- disc & 0 & / & 854 & (0.00\%) & 589 & / & 854 & (68.97\%) & 745 & / & 854 & (87.24\%) & 745 & / & 854 & (87.24\%) & 757 & / & 854 & (88.64\%)\\
\hline
& Total time (min)& \multicolumn{4}{|r}{0.000383333}& \multicolumn{4}{|r}{0.0429167}& \multicolumn{4}{|r}{0.119}& \multicolumn{4}{|r}{0.293883}& \multicolumn{4}{|r}{0.340133}\\
& Sentences / min& \multicolumn{4}{|r}{6302610.0}& \multicolumn{4}{|r}{56295.1}& \multicolumn{4}{|r}{20302.5}& \multicolumn{4}{|r}{8220.95}& \multicolumn{4}{|r}{7103.1}\\
& Tokens / min& \multicolumn{4}{|r}{147871000.0}& \multicolumn{4}{|r}{1320790.0}& \multicolumn{4}{|r}{476336.0}& \multicolumn{4}{|r}{192879.0}& \multicolumn{4}{|r}{166652.0}\\
\hline
\hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{negra (dev)}}}
& bd2 & 6795 & / & 7145 & (95.10\%) & 7081 & / & 7145 & (99.10\%) & 7135 & / & 7145 & (99.86\%) & 7135 & / & 7145 & (99.86\%) & 7145 & / & 7145 & (100.00\%)\\
&- disc & 0 & / & 350 & (0.00\%) & 286 & / & 350 & (81.71\%) & 340 & / & 350 & (97.14\%) & 340 & / & 350 & (97.14\%) & 350 & / & 350 & (100.00\%)\\
& all & 6795 & / & 7191 & (94.49\%) & 7081 & / & 7191 & (98.47\%) & 7135 & / & 7191 & (99.22\%) & 7135 & / & 7191 & (99.22\%) & 7145 & / & 7191 & (99.36\%)\\
&- disc & 0 & / & 396 & (0.00\%) & 286 & / & 396 & (72.22\%) & 340 & / & 396 & (85.86\%) & 340 & / & 396 & (85.86\%) & 350 & / & 396 & (88.38\%)\\
\hline
& Total time (min)& \multicolumn{4}{|r}{8.33333e-05}& \multicolumn{4}{|r}{0.00693333}& \multicolumn{4}{|r}{0.02035}& \multicolumn{4}{|r}{0.0449167}& \multicolumn{4}{|r}{0.0501833}\\
& Sentences / min& \multicolumn{4}{|r}{12000000.0}& \multicolumn{4}{|r}{144231.0}& \multicolumn{4}{|r}{49140.1}& \multicolumn{4}{|r}{22263.5}& \multicolumn{4}{|r}{19926.9}\\
& Tokens / min& \multicolumn{4}{|r}{208728000.0}& \multicolumn{4}{|r}{2508750.0}& \multicolumn{4}{|r}{854742.0}& \multicolumn{4}{|r}{387250.0}& \multicolumn{4}{|r}{346609.0}\\
\hline
\hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{negra (test)}}}
& bd2 & 6404 & / & 6808 & (94.07\%) & 6732 & / & 6808 & (98.88\%) & 6798 & / & 6808 & (99.85\%) & 6798 & / & 6808 & (99.85\%) & 6808 & / & 6808 & (100.00\%)\\
&- disc & 0 & / & 404 & (0.00\%) & 328 & / & 404 & (81.19\%) & 394 & / & 404 & (97.52\%) & 394 & / & 404 & (97.52\%) & 404 & / & 404 & (100.00\%)\\
& all & 6404 & / & 6842 & (93.60\%) & 6732 & / & 6842 & (98.39\%) & 6798 & / & 6842 & (99.36\%) & 6798 & / & 6842 & (99.36\%) & 6808 & / & 6842 & (99.50\%)\\
&- disc & 0 & / & 438 & (0.00\%) & 328 & / & 438 & (74.89\%) & 394 & / & 438 & (89.95\%) & 394 & / & 438 & (89.95\%) & 404 & / & 438 & (92.24\%)\\
\hline
& Total time (min)& \multicolumn{4}{|r}{8.33333e-05}& \multicolumn{4}{|r}{0.00876667}& \multicolumn{4}{|r}{0.0249167}& \multicolumn{4}{|r}{0.0606333}& \multicolumn{4}{|r}{0.0707333}\\
& Sentences / min& \multicolumn{4}{|r}{12000000.0}& \multicolumn{4}{|r}{114068.0}& \multicolumn{4}{|r}{40133.8}& \multicolumn{4}{|r}{16492.6}& \multicolumn{4}{|r}{14137.6}\\
& Tokens / min& \multicolumn{4}{|r}{200904000.0}& \multicolumn{4}{|r}{1909730.0}& \multicolumn{4}{|r}{671920.0}& \multicolumn{4}{|r}{276119.0}& \multicolumn{4}{|r}{236692.0}\\
\hline
\hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{tiger spmrl (dev)}}}
& bd2 & 30930 & / & 32416 & (95.42\%) & 32181 & / & 32416 & (99.28\%) & 32374 & / & 32416 & (99.87\%) & 32374 & / & 32416 & (99.87\%) & 32416 & / & 32416 & (100.00\%)\\
&- disc & 0 & / & 1486 & (0.00\%) & 1251 & / & 1486 & (84.19\%) & 1444 & / & 1486 & (97.17\%) & 1444 & / & 1486 & (97.17\%) & 1486 & / & 1486 & (100.00\%)\\
& all & 30930 & / & 32578 & (94.94\%) & 32181 & / & 32578 & (98.78\%) & 32374 & / & 32578 & (99.37\%) & 32374 & / & 32578 & (99.37\%) & 32416 & / & 32578 & (99.50\%)\\
&- disc & 0 & / & 1648 & (0.00\%) & 1251 & / & 1648 & (75.91\%) & 1444 & / & 1648 & (87.62\%) & 1444 & / & 1648 & (87.62\%) & 1486 & / & 1648 & (90.17\%)\\
\hline
& Total time (min)& \multicolumn{4}{|r}{0.000366667}& \multicolumn{4}{|r}{0.0230833}& \multicolumn{4}{|r}{0.0672333}& \multicolumn{4}{|r}{0.16155}& \multicolumn{4}{|r}{0.18265}\\
& Sentences / min& \multicolumn{4}{|r}{13636400.0}& \multicolumn{4}{|r}{216606.0}& \multicolumn{4}{|r}{74367.9}& \multicolumn{4}{|r}{30950.2}& \multicolumn{4}{|r}{27374.8}\\
& Tokens / min& \multicolumn{4}{|r}{209193000.0}& \multicolumn{4}{|r}{3322920.0}& \multicolumn{4}{|r}{1140860.0}& \multicolumn{4}{|r}{474800.0}& \multicolumn{4}{|r}{419951.0}\\
\hline
\hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{tiger spmrl (test)}}}
& bd2 & 36079 & / & 38041 & (94.84\%) & 37686 & / & 38041 & (99.07\%) & 37991 & / & 38041 & (99.87\%) & 37991 & / & 38041 & (99.87\%) & 38039 & / & 38041 & (99.99\%)\\
&- disc & 0 & / & 1962 & (0.00\%) & 1607 & / & 1962 & (81.91\%) & 1912 & / & 1962 & (97.45\%) & 1912 & / & 1962 & (97.45\%) & 1960 & / & 1962 & (99.90\%)\\
& all & 36079 & / & 38235 & (94.36\%) & 37686 & / & 38235 & (98.56\%) & 37991 & / & 38235 & (99.36\%) & 37991 & / & 38235 & (99.36\%) & 38039 & / & 38235 & (99.49\%)\\
&- disc & 0 & / & 2156 & (0.00\%) & 1607 & / & 2156 & (74.54\%) & 1912 & / & 2156 & (88.68\%) & 1912 & / & 2156 & (88.68\%) & 1960 & / & 2156 & (90.91\%)\\
\hline
& Total time (min)& \multicolumn{4}{|r}{0.00065}& \multicolumn{4}{|r}{0.150967}& \multicolumn{4}{|r}{0.71085}& \multicolumn{4}{|r}{4.34097}& \multicolumn{4}{|r}{4.68583}\\
& Sentences / min& \multicolumn{4}{|r}{7692310.0}& \multicolumn{4}{|r}{33119.9}& \multicolumn{4}{|r}{7033.83}& \multicolumn{4}{|r}{1151.82}& \multicolumn{4}{|r}{1067.05}\\
& Tokens / min& \multicolumn{4}{|r}{141545000.0}& \multicolumn{4}{|r}{609433.0}& \multicolumn{4}{|r}{129428.0}& \multicolumn{4}{|r}{21194.4}& \multicolumn{4}{|r}{19634.5}\\
\hline
\hline
\end{tabular}

==> table/recall.tex <==
\begin{tabular}{l|l|c|c|c|c|c}
 & & \multicolumn{1}{|c}{Continuous} & \multicolumn{1}{|c}{N4} & \multicolumn{1}{|c}{N5} & \multicolumn{1}{|c}{Well-nested} & \multicolumn{1}{|c}{Ill-nested} \\
 \hline
 \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{dptb}}}
 & bd2& 98.2\%& 99.6\%& 100.0\%& 100.0\%& 100.0\%\\
 &- disc& 0.0\%& 77.8\%& 98.4\%& 98.4\%& 100.0\%\\
 & all& 98.0\%& 99.4\%& 99.7\%& 99.7\%& 99.8\%\\
 &- disc& 0.0\%& 69.0\%& 87.2\%& 87.2\%& 88.6\%\\
 \hline
 \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{negra}}}
 & bd2& 94.1\%& 98.9\%& 99.9\%& 99.9\%& 100.0\%\\
 &- disc& 0.0\%& 81.2\%& 97.5\%& 97.5\%& 100.0\%\\
 & all& 93.6\%& 98.4\%& 99.4\%& 99.4\%& 99.5\%\\
 &- disc& 0.0\%& 74.9\%& 90.0\%& 90.0\%& 92.2\%\\
 \hline
 \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{tiger}}}
 & bd2& 94.8\%& 99.1\%& 99.9\%& 99.9\%& 100.0\%\\

 &- disc& 0.0\%& 81.9\%& 97.5\%& 97.5\%& 99.9\%\\
 & all& 94.4\%& 98.6\%& 99.4\%& 99.4\%& 99.5\%\\
 &- disc& 0.0\%& 74.5\%& 88.7\%& 88.7\%& 90.9\%\\
 \hline
 \end{tabular}

